Spatially parallel decoding for multi-qubit lattice surgery

Running quantum algorithms protected by quantum error correction requires a real time, classical decoder. To prevent the accumulation of a backlog, this decoder must process syndromes from the quantum device at a faster rate than they are generated. Most prior work on real time decoding has focused on an isolated logical qubit encoded in the surface code. However, for surface code, quantum programs of utility will require multi-qubit interactions performed via lattice surgery. A large merged patch can arise during lattice surgery -- possibly as large as the entire device. This puts a significant strain on a real time decoder, which must decode errors on this merged patch and maintain the level of fault-tolerance that it achieves on isolated logical qubits. These requirements are relaxed by using spatially parallel decoding, which can be accomplished by dividing the physical qubits on the device into multiple overlapping groups and assigning a decoder module to each. We refer to this approach as spatially parallel windows. While previous work has explored similar ideas, none have addressed system-specific considerations pertinent to the task or the constraints from using hardware accelerators. In this work, we demonstrate how to configure spatially parallel windows, so that the scheme (1) is compatible with hardware accelerators, (2) supports general lattice surgery operations, (3) maintains the fidelity of the logical qubits, and (4) meets the throughput requirement for real time decoding. Furthermore, our results reveal the importance of optimally choosing the buffer width to achieve a balance between accuracy and throughput -- a decision that should be influenced by the device's physical noise.

==> sections/cover_page.tex <==
\setcounter{page}{0}
Thank you for your helpful feedback. We will give a summary of the revisions, then address some of the specific questions.

\noindent\textbf{Revisions:} The changes in (1) are highlighted in \hlc{yellow} and the rest are highlighted in \hlc[pink]{pink}.
\begin{enumerate}
    \item Improved the writing based on the feedback from reviewers A, C, D (e.g. we split Fig. 3 into 2 cases and added labels to Fig. 4), and more accurately described Skoric et al. following reviewer B’s suggestion. We also made a lot of other writing changes that are not highlighted.
    \item Added simulations with 2D window configurations since reviewers D and E pointed out that results beyond the simple two-window configuration would be helpful. We found that the case where a thicker patch is divided into multiple rows of windows does not require larger buffer than already required by the narrow long patch.
    \item Improved the discussion of throughput and latency, including:
    \begin{itemize}
        \item elaborated on the impact of throughput and latency on performance (Section 4B).
        \item restructured and expanded Section 6. We separated the content on inter-window communication and the inner decoder into two subsections, and added more information and discussion on inner decoders.
    \end{itemize}
\end{enumerate}
\textbf{Clarifications and responses to specific questions:}

\noindent\textbf{Cost of serialization (E):} We want to clarify this. When the window size is fixed, the cost of serialization (in terms of total latency) is proportional to the number of layers that the windows are divided into (which is constant --- 2 or 3), rather than the number of windows that a long patch spans. Thus, the latency of the parallel windows does not depend on the length of a long patch. We have a more detailed discussion of latency and its impact in the revised draft.

\noindent\textbf{Code threshold (C):} The threshold is the physical error $p$, such that when the noise on a device is below $p$, one can suppress the logical error rate by increasing the code distance. Fig 8 shows that when the buffer is big enough, the logical error rate from windowed decoding is very close to the one from global decoding (the difference is negligible compared to the global decoder’s logical error rate at larger or smaller distances when $p$ is below threshold). Therefore, we don’t expect windowed decoding to change the threshold.

\noindent\textbf{Limit of monolithic decoders \& need for spatial parallelism (D \& E):} The scalability challenge of monolithic decoders is not due to FPGA, but is inherent to the decoding problem. The complexity of decoding algorithms is expressed in terms of n, the number of nodes in the decoding graph ($\sim$\# of physical qubits $\times$ \# of measurement cycles). The STOA MWPM software decoder (PyMatching2) has an $O(n)$ empirical runtime, which is quite ideal for a monolithic decoder. Even the UF algorithm, simpler than MWPM, has a theoretical complexity that is slightly more than linear. This is why we say the cost of a monolithic decoder grows at least linearly with the length of a patch. \textbf{E} pointed out that the reported empirical runtime of decoders might come from using only square patches, so we ran PyMatching2 on $7\times n$ rectangular patches (each shot uses 7 measurements rounds) on a laptop with $p=0.2\%$, and confirmed that the linear scaling also holds for long rectangular patches (see Fig. \ref{fig:global_runtime} on the cover page). We only count the time for decoding and exclude the time for sampling, but since we are not using a timer inside the decoder package, we might have included a boot time (which does not depend on the patch size so it doesn't affect our conclusion on the scaling).
\begin{figure}
  \centering
  \includegraphics[scale=0.4]{figs/global_runtime.pdf}
  \caption{Runtime of PyMatching2 on a $7\times n\times7$ decoding graph. The plot shows the total time for 2M shots.}
  \label{fig:global_runtime}
\end{figure}

\noindent\textbf{Capacity of one FPGA (C \& D):} We consider the case where each FPGA performs decoding on one window, instead of fitting multiple windows on 1 FPGA or using multiple FPGAs for 1 window. 

The parallel scheme in this paper can help with demonstrations of logical operations, which can involve many logical qubits across the device. Thus we don't think all windows can be implemented on the same FPGA. 

We don't use multiple FPGAs for each window because, as mentioned in the revised paper, FPGA decoders typically use shared memory for communication. If an inner decoder is spread on multiple FPGAs, it will run much slower due to the increased communication cost. Furthermore, the inner decoders that fit on 1 FPGA have enough capacity for medium-sized patches. For larger sizes, one can move to ASICs that are more efficient. Also note that very large window sizes are not needed, because the logical error rate is exponentially suppressed with the code distance, e.g. it suffices to use $d=27$ for Shor's algorithm with 2048 bit integers~\cite{gidney2021factor}, which is considered a very large program that require millions of physical qubits.

\noindent\textbf{B’s last question:} Fig. 8 actually shows that at a tiny buffer width like 2, buffered error correction can have $>100$X higher logical error than global, at small $p$.

\noindent\textbf{Why FPGA implementation or synthesis is not included (B):} Our work is not on a new inner decoder, but rather how they should be connected. Therefore, the performance of the scheme can be computed given the data about the inner decoder and the window setup. We hope the new version gives a better explanation of how this is done.
\setcounter{figure}{0}
